Quantum Advantage from Any Non-Local Game

We show a general method of compiling any $k$-prover non-local game into a single-prover interactive game maintaining the same (quantum) completeness and (classical) soundness guarantees (up to negligible additive factors in a security parameter). Our compiler uses any quantum homomorphic encryption scheme (Mahadev, FOCS 2018; Brakerski, CRYPTO 2018) satisfying a natural form of correctness with respect to auxiliary (quantum) input. The homomorphic encryption scheme is used as a cryptographic mechanism to simulate the effect of spatial separation, and is required to evaluate $k-1$ prover strategies (out of $k$) on encrypted queries. In conjunction with the rich literature on (entangled) multi-prover non-local games starting from the celebrated CHSH game (Clauser, Horne, Shimonyi and Holt, Physical Review Letters 1969), our compiler gives a broad framework for constructing mechanisms to classically verify quantum advantage.

==> notes.tex <==

\lisa{%\section{Things to Think About}
\begin{itemize}
    \item Can we get efficient protocol (without security parameter)? Is there a nonlocal game where one prover applies Clifford gates?
\end{itemize}}

\lisa{First, working on the basic protocol. Looking ahead:}

\lisa{Is small soundness/1-eps difference between the success of classical vs quantum computers desired? If so, seems need some repetition; need to be careful about the efficiency. Maybe just run protocol sequentially if repetitions small enough.}

\vinod{Yes, I would come up with a protocol with constant gap. That's sufficient to show quantum advantage.}

\lisa{Can quantum computers prepare maximally entangled states or only approximately? May want to ask someone what abstract to work with; we may need to consider approx max entangled states.}

\vinod{Good question, I think we should ignore this ``engineering concern'' for now. But I also think you can approximate arbitrarily (up to trace distance $\epsilon$) with circuits of size $\log 1/\epsilon$.}

\lisa{Rough thought: Is there some notion of a 'computational Bell inequality'/entanglement measure in the prover's state needing to be high (i.e. the prover has to be quantum) be obtained in this compilation, and/or shown to be underneath quantum supremacy protocols.}

